Flare Prediction Using Photospheric and Coronal Image Data

The precise physical process that triggers solar flares is not currently understood. Here we attempt to capture the signature of this mechanism in solar image data of various wavelengths and use these signatures to predict flaring activity. We do this by developing an algorithm that [1] automatically generates features in 5.5 TB of image data taken by the Solar Dynamics Observatory of the solar photosphere, chromosphere, transition region, and corona during the time period between May 2010 and May 2014, [2] combines these features with other features based on flaring history and a physical understanding of putative flaring processes, and [3] classifies these features to predict whether a solar active region will flare within a time period of $T$ hours, where $T$ = 2 and 24. We find that when optimizing for the True Skill Score (TSS), photospheric vector magnetic field data combined with flaring history yields the best performance, and when optimizing for the area under the precision-recall curve, all the data are helpful. Our model performance yields a TSS of $0.84 \pm 0.03$ and $0.81 \pm 0.03$ in the $T$ = 2 and 24 hour cases, respectively, and a value of $0.13 \pm 0.07$ and $0.43 \pm 0.08$ for the area under the precision-recall curve in the $T$ = 2 and 24 hour cases, respectively. These relatively high scores are similar to, but not greater than, other attempts to predict solar flares. Given the similar values of algorithm performance across various types of models reported in the literature, we conclude that we can expect a certain baseline predictive capacity using these data. This is the first attempt to predict solar flares using photospheric vector magnetic field data as well as multiple wavelengths of image data from the chromosphere, transition region, and corona.

==> Makefile <==

PDFLATEX=/usr/local/texlive/2017/bin/x86_64-darwin/pdflatex
BIBTEX=/usr/local/texlive/2017/bin/x86_64-darwin/bibtex

BIBSRC = /Users/jonas/Documents/Bibtex/solar\ physics.bib

all: predict.pdf

getbib: ${BIBSRC}
	cp ${BIBSRC} jonas.bib

predict.pdf: predict.tex
	${PDFLATEX} predict.tex
	${BIBTEX} predict
	${PDFLATEX} predict.tex

clean:
	rm -Rf predict.aux predict.bbl predict.blg predict.log predict.lox predict.toc predict.pdf

